Short-term variations of surface magnetism and prominences of the young Sun-like star V530 Per

Aims: We investigate magnetic tracers in the photosphere and the chromosphere of the ultra-rapid rotator ($P\sim0.32d$) V530 Per, a cool member of the open cluster $\alpha$ Persei, to characterize the short-term variability of the magnetic activity and large-scale magnetic field of this prototypical young, rapidly rotating solar-like star. Methods: With time-resolved spectropolarimetric observations spread over four close-by nights, we reconstructed the brightness distribution and large-scale magnetic field geometry of V530 Per through Zeeman-Doppler imaging. Simultaneously, we estimated the short-term variability of the surface through latitudinal differential rotation. Using the same data set, we also mapped the spatial distribution of prominences through tomography of H$\alpha$ emission. Results: As in our previous study, a large dark spot occupies the polar region of V530 Per with smaller, dark, and bright spots at lower latitudes. The large-scale magnetic field is dominated by a toroidal, mostly axisymmetric component. The maximal radial field strength is equal to $\sim1$ kG. The surface differential rotation is consistent with a smooth Sun-like shear d$\Omega = 0.053 \pm 0.004$ rad.d$^{-1}$, close to the solar shear level. The prominence pattern displays a stable component that is confined close to the corotation radius. We also observe rapidly evolving H$\alpha$ emitting structures, over timescales ranging from minutes to days. The fast H$\alpha$ evolution was not linked to any detected photospheric changes in the spot or magnetic coverage.

==> Tables/AllTab.tex <==
%----------> tab:obslog <-----------% 
\input{Tables/obslog}
\input{Tables/Parameters}
\input{Tables/magE.tex}

==> Tables/Parameters.tex <==
% Table that lists all parameters

\begin{table}[h]

\caption{Parameters of AP 149}
          \centering
          \begin{tabular}{l|l|l}
        \hline
 Name & Values&  References\\ 
\hline
Distance & $167.7\pm15$ pc& 1,2\\
Age  &$33^{+10}_{-7}$~Myr& 1 \\
$T_\mathrm{eff}$ &$5281\pm96$ K& 1\\
log$~g$ &$4.1 \pm 0.19$ & 1\\
$[Fe/H]$ & 0 & 1\\
$m_V^{max}$ &$11.657\pm0.13$&4\\
$m_K$  &$9.422 \pm0.019 $& 4 \\
$m_J$ & $10.08 \pm 0.019 $ & 4 \\
Luminosity & $0.76 \pm 0.18~L_{\sun}$ &1\\
Radius & $1.04 \pm 0.11~R_{\sun}$ & 1 \\
Mass & $1.03\pm0.13$~$M_{\sun}$ &  1 \\
$log~L_{x}$ & 31.2 &5\\
Rossby number &$0.0128 \pm0.0019$& 1\\
Co-rotation radius &$1.92~R_{*}$& 1\\
\vsini & $105.6~\kms $ & 1  \\
Eq. rot. period &$0.3205 \pm 0.0002$~d& 1\\
$d\Omega$ &$0.043 \pm 0.007$~\rpd& 1\\
Inclination angle &$35\pm0.2^{\circ}$ & 1 \\
Radial velocity  & $-0.96\pm0.04~\kms $ & 1 \\
        \hline
        \end{tabular}
\textbf{\tt{References: }}~1. This work 2. \cite{2018A&A...615A..12Y} 3. \cite{1999ApJ...527..219S}  4. \cite{2012yCat.1322....0Z} 5. \cite{2013AJ....145..143P}
\label{tab:para}
\end{table}
%-----------------------------------------%

==> Tables/magE.tex <==
\begin{table}[]
    \centering
    \caption{Magnetic field characteristics of AP 149. The values include (a) the average magnetic field strength $\langle B \rangle$, (b) the unsigned peak magnetic field strength $|B_{peak}|$, (c) the ratio of toroidal field energy with respect to the total magnetic energy, (d) the ratio of magnetic energy in axisymmetric modes ($m = 0$) over the total energy, the same quantity but limited to the poloidal (e) and toroidal (f) magnetic component, the ratio of the dipole, quadrupole, and octopole (g, h, i) as a fraction of the poloidal component, and ($\ell=1,2,3$) subcomponents of the toroidal field energy, as a fraction of the toroidal field energy (j, k, and l).}
    \begin{tabular}{l|l}
        \hline
        $\langle B \rangle$  & 155 G \\
        $|B_{peak}|$  & 1019 G\\
        Toroidal & 67  \%  (total)\\
        axisymmetric  & 54 \% (total)\\
        poloidal axisymmetric  & 15 \% (poloidal)\\
        toroidal axisymmetric  & 74 \% (toroidal)\\
        dipole  & 1.1 \% (poloidal)\\
        quadrupole  & 3.0 \% (poloidal)\\
        octopole  & 4.8 \% (poloidal)\\
        {\newm poloidal $\ell > 3$ & 91.1 (poloidal) \%} \\
        toroidal $\ell = 1$  & 5.1 \% (toroidal)\\
        toroidal $\ell = 2$  & 17 \% (toroidal)\\
        toroidal $\ell = 3$ & 19 \% (toroidal)\\
        {\newm toroidal $\ell > 3$ & 58.9 \% (toroidal)}\\
        \hline
        
    \end{tabular}
    \label{tab:magE}
\end{table}

% Bmean =   154.862 G
% Bmax =   1018.612 G
% poloidal 33.334% (% tot)
% toroidal 66.666% (% tot)
% dipole:  1.120% (% pol)
% quadrupole:  2.986% (% pol)
% octopole:  4.761% (% pol)
% toroidal l1:  5.124% (% tor)
% toroidal l2: 16.782% (% tor)
% toroidal l3: 19.398% (% tor)
% axisymmetric: 54.093% (% tot)
% poloidal axisymmetric: 15.374% (% pol)
% toroidal axisymmetric: 73.453% (% tor)
% dipol axisymmetric: 22.252% (% dip)
% Dipolar max =     22.425 G, colat   58.5 long  151.9
% Dipole radial + pole =     21.386 G, colat   58.5 long  149.5
% Dipole radial - pole =    -21.387 G, colat  121.5 long  330.1

